NeuralExplorer: State Space Exploration of Closed Loop Control Systems Using Neural Networks

In this paper, we propose a framework for performing state space exploration of closed loop control systems. Our approach involves approximating sensitivity and a newly introduced notion of inverse sensitivity by a neural network. We show how the approximation of sensitivity and inverse sensitivity can be used for computing estimates of the reachable set. We then outline algorithms for performing state space exploration by generating trajectories that reach a neighborhood. We demonstrate the effectiveness of our approach by applying it not only to standard linear and nonlinear dynamical systems, but also to nonlinear hybrid systems and also neural network based feedback control systems.

==> psd-macros.tex <==
\usepackage{tikz}
\usepackage[usenames,dvipsnames]{pstricks}
%\usepackage{epsfig} -- here

%\usepackage{palatino}
\RequirePackage{ifthen}
% \RequirePackage{amsmath}
% \RequirePackage{amssymb}
\RequirePackage{listings}
\RequirePackage{mathrsfs}
\RequirePackage{xspace}
\RequirePackage{graphics}

% PACKAGES FOR ORGANIZING THE STRUCTE OF DOCUMENT
%\usepackage{minipage}
\usepackage{latexsym}
\usepackage{multicol}
\usepackage{multirow}
\usepackage{lscape}  % Useful for wide tables or figures.
\usepackage{xspace}
\usepackage{paralist}
%\usepackage{framed}
%\usepackage{lipsum}
% DEFINING THE BOUNDARY --- DONE IN DOCUMENT.
%\usepackage[left=1.25in,right=1.25in,top=1in,bottom=1.25in]{geometry}

%%% SECTION TITLE APPEARANCE
% \usepackage{sectsty}
% \allsectionsfont{\sffamily\mdseries\upshape} % (See the fntguide.pdf for font help)
% (This matches ConTeXt defaults)

%%% HEADERS & FOOTERS
% \usepackage{fancyhdr} % This should be set AFTER setting up the page geometry
% \pagestyle{fancy} % options: empty , plain , fancy
% \renewcommand{\headrulewidth}{0pt} % customise the layout...
% \lhead{}\chead{}\rhead{}
% \lfoot{}\cfoot{\thepage}\rfoot{}


% PACKAGES FOR FIGURES
\usepackage{xcolor}
\usepackage{float}
%\usepackage{subfigure} -- here
\usepackage{subfloat}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{wrapfig}
%\usepackage{pifont}
%\usepackage{subcaption}
%\usepackage{subfigure}  % for subfigures
%\usepackage{setspace}
%\usepackage[justification=raggedright]{caption}	% makes captions ragged right - thanks to Bryce Lobdell

%AMS AND OTHER MISC PACKAGES
\usepackage{keyval}
\usepackage{amsmath,amssymb,amsfonts,url,listings,mathrsfs}
%reference
%\usepackage[pdftex,colorlinks,citecolor=webblue,linkcolor=webblue,urlcolor=webblue]{hyperref} -- here

%ALGORITHM PACKAGE
%\usepackage{algorithm,algorithmic}
%
%\usepackage[pdftex,colorlinks,citecolor=webblue,linkcolor=webred,backref,pagebackref]{hyperref}
%\usepackage[linesnumbered,lined,commentsnumbered]{algorithm2e}
%\usepackage[linesnumbered,boxed,lined,commentsnumbered,algochapter]{algorithm2e}


%DEFINITIONS FOR MARKING CHANGES AND COMMENTS
\newcommand{\authcomment}[1]{\textbf{[[#1]]}}
%\newcommand{\sayan}[1]{\textcolor{blue}{[[#1]]}}
%\newcommand{\sridhar}[1]{\textcolor{red}{[[#1]]}}
\newcommand{\sridhar}[1]{\textcolor{brown}{[[#1]]}}

% DEFINING COLORS
\definecolor{reddish}{rgb}{1,.8,0.8}
\definecolor{blueish}{rgb}{0.8,.8,1}
\definecolor{greenish}{rgb}{.8,1,0.8}
\definecolor{yellowish}{rgb}{1,1,.20}
\definecolor{webred}{rgb}{0.5,0,0}
\definecolor{webblue}{rgb}{0,0,0.8}

% DEFINITIONS FOR TEXT FORMATTING
\newcommand{\figuresize}{\scriptsize}
\newcommand{\equationsize}{\footnotesize}

% ADHOC DEFINITIONS FOR EACH AND EVERY PAPER
\newcommand{\trajmet}{discrepancy function\/}
\newcommand{\TrajMet}{Trajectory Metric}
\newcommand{\RT}{{\em reachtubes}}
\newcommand{\valsim}{{\sf valSim}}
\newcommand{\tool}{C2E2 \/}
\newcommand{\fulltoolname}{\textbf{C}heck \textbf{E}xecute \textbf{C}ompare \textbf{E}ngine}
\newcommand{\leftshift}[2]{\relax\ifmmode (#1 \lhd #2) \else $(#1 \lhd #2)$ \fi}
\newcommand{\mayInt}{\relax\ifmmode \mathit{mayInt} \else $\mathit{mayInt}$ \fi}
\newcommand{\mustInt}{\relax\ifmmode \mathit{mustInt} \else $\mathit{mustInt}$ \fi}
\newcommand{\notInt}{\relax\ifmmode \mathit{notInt} \else $\mathit{notInt}$ \fi}
\newcommand{\alarm}{\relax\ifmmode \mathit{Alert} \else $\mathit{Alert}$ \fi}
\newcommand{\unsafe}{\relax\ifmmode \mathit{Unsafe} \else $\mathit{Unsafe}$ \fi}
\newcommand{\xsep}{\relax\ifmmode \mathit{xsep} \else $\mathit{xsep}$\fi}
\newcommand{\ysep}{\relax\ifmmode \mathit{ysep} \else $\mathit{ysep}$ \fi}
\newcommand{\etime}{{\sf time}}
\newcommand{\ub}{{\sf ub}}
\newcommand{\lb}{{\sf lb}}
\newcommand{\emode}{{\sf mode}}
\newcommand{\erange}{{\sf range}}
\newcommand{\fbls} {functionally bounded linear span}
\newcommand{\fblsupper} {Functionally bounded linear span}

% COMMANDS USED IN DEFINITIONS
\newcommand{\meansl}{[\![}
\newcommand{\meansr}{]\!]}
\newcommand{\means}[1]{\meansl #1 \meansr}
\newcommand{\Nset}[1]{[[#1]]}

% ROUTINELY USED COMMANDS
\newcommand{\refinement}[1]{\relax\ifmmode \mathit{refine}(#1) \else $\mathit{refine}(#1)$ \fi}
\newcommand{\diff}{{\sf diff}}
\newcommand{\diameter} {\mathsf{diameter}}
\newcommand{\cntr} {\mathsf{center}}
\newcommand{\ball}[1] {B_{#1}}
\newcommand{\true}{\relax\ifmmode \mathit true \else \em true \/\fi}
\newcommand{\false}{\relax\ifmmode \mathit false \else \em false \/\fi}
% \newcommand{\lnot}{\neg} % Already defined
% \newcommand{\land}{\wedge} % Already defined
% \newcommand{\lor}{\vee} % Already defined
\newcommand{\limplies}{\Rightarrow}
\newcommand{\liff}{\Leftrightarrow}
%\newcommand{\T}{\mathit{true}}
%\newcommand{\F}{\mathit{false}}
% \newcommand{\to}{\relax\ifmmode \rightarrow \else $\rightarrow$\fi} % Already defined
\newcommand{\fro}{\relax\ifmmode \leftarrow \else $\leftarrow$\fi}


% COMMANDS FOR MATH SPECIFIC ITEMS
\newcommand{\nnt}{{\sf T}^{\geq 0}}             %nonnegative time points
\newcommand{\post}{{\sf T}^{>0}}                %positive time points
\newcommand{\Variables}{{\sf V}}                %variables

\newcommand{\num}[1]{\relax\ifmmode \mathbb #1\else $\mathbb #1$\fi}
\newcommand{\nnnum}[1]{\relax\ifmmode 
  {\mathbb #1}_{\geq 0} \else ${\mathbb #1}_{\geq 0}$
  \fi}
\newcommand{\npnum}[1]{\relax\ifmmode 
  {\mathbb #1}_{\leq 0} \else ${\mathbb #1}_{\leq 0}$
  \fi}
\newcommand{\pnum}[1]{\relax\ifmmode 
  {\mathbb #1}_{> 0} \else ${\mathbb #1}_{> 0}$
  \fi}
\newcommand{\nnum}[1]{\relax\ifmmode 
  {\mathbb #1}_{< 0} \else ${\mathbb #1}_{< 0}$
  \fi}
\newcommand{\plnum}[1]{\relax\ifmmode 
  {\mathbb #1}_{+} \else ${\mathbb #1}_{+}$
  \fi}
\newcommand{\nenum}[1]{\relax\ifmmode 
  {\mathbb #1}_{-} \else ${\mathbb #1}_{-}$
  \fi}

\newcommand{\reals}{{\num R}}                    %reals
\newcommand{\nnreals}{{\nnnum R}}                    %nonnegative reals
\newcommand{\realsinfty}{{\num R} \cup \{\infty, -\infty\}}                    %nonnegative reals
\newcommand{\plreals}{{\plnum R}}                    %positive reals
\newcommand{\naturals}{{\num N}}                      %natural numbers
\newcommand{\integers}{{\num Z}}                      %integers
\newcommand{\rationals}{{\num Q}}                      %rationals
\newcommand{\nnrationals}{{\nnnum Q}}                   % nonnegative rationals
\newcommand{\Time}{{\num T}}  
\newcommand{\bools}{{\num B}}  
\newcommand{\plintegers}{{\plnum Z}}                      %integers
\newcommand{\deq}{\mathrel{\stackrel{\scriptscriptstyle\Delta}{=}}}
\newcommand{\intervals}{\relax \ifmmode \mathbb{IR} \else $\mathbb{IR}$ \fi}
\newcommand{\nnintervals}{\relax \ifmmode \mathbb{IR}^{+} \else $\mathbb{IR}^{+}$ \fi}
%\setlength{\mathindent}{0pt}

% COMMANDS FOR LABELS
\renewcommand{\eqref}[1]{Equation~(\ref{eq:#1})}
\newcommand{\eqlabel}[1]{\label{eq:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\figrefs}[2]{Figures~\ref{fig:#1} and~\ref{fig:#2}}
\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{table:#1}}
\newcommand{\tablabel}[1]{\label{table:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\deflabel}[1]{\label{def:#1}}
\newcommand{\exref}[1]{Example~\ref{exmp:#1}}
\newcommand{\exlabel}[1]{\label{exmp:#1}}
\newcommand{\scref}[1]{Section~\ref{sec:#1}}
\newcommand{\secreftwo}[2]{Sections~\ref{sec:#1}~and~\ref{sec:#2}}
\newcommand{\sclabel}[1]{\label{sec:#1}}
\newcommand{\applabel}[1]{\label{app:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
\newcommand{\lnlabel}[1]{\label{line:#1}}
\newcommand{\lnrngref}[2]{lines~\ref{line:#1}--\ref{line:#2}\xspace}
\newcommand{\lnref}[1]{line~\ref{line:#1}\xspace}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}\xspace}
%\newcommand{\seclabel}[1]{\label{sec:#1}}
%\newcommand{\secref}[1]{Section~\ref{sec:#1}}
%\newcommand{\figlabel}[1]{\label{fig:#1}}
%\newcommand{\figref}[1]{Figure~\ref{fig:#1}}


% COMMANDS FOR SECTIONS AND ORGANIZATION

\newenvironment{noqedproof}{\pf}{}
\newcommand{\pf}{\par\noindent{\bf Proof:}~}
% \newcounter{theorem}
% \setcounter{theorem}{0}
% 
%  \newtheorem{theorem}{Theorem}
%  \newtheorem{lemma}[theorem]{Lemma}
%  \newtheorem{corollary}[theorem]{Corollary}
%  \newtheorem*{claim}{Claim}
%  \newtheorem{assumption}{Assumption}
%  \theoremstyle{definition}
%  \newtheorem{definition}{Definition}
%  \newcommand{\qed}{\hfill{\rule{2mm}{2mm}}\medskip}
%  \newenvironment{proof}{\pf}{\qed}
%  \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{inv}[theorem]{Invariant}
 
%    \newcounter{rem}
%  \setcounter{rem}{0}
%  
%   \newenvironment{remark}
%   {\refstepcounter{rem} \vspace{2ex}\par\noindent
%    \textbf{Remark}~\textbf{\therem~}}
 
% \newcounter{example}
%  \setcounter{example}{0}

%   \newtheorem{example}[example]{Example}
%  \newcounter{example}
  
%  \newenvironment{example}
%  {\refstepcounter{example} \vspace{2ex}\par\noindent
%  \textbf{Example}~\textbf{\theexample~}}%{\qed}
% \newexample{example}[example]{Example}

%\theoremstyle{remark}
%\newcounter{example}
% \newtheorem{example}{Example}[chapter]
% {\refstepcounter{theorem} \vspace{2ex}\par\noindent
% \textbf{Example}~\textbf{\theexampletheorem~}}{\qed}
 
 \def\examplenonum#1#2{
        \vspace{.15in}
        \noindent
        {\bf Example #1}{\em ~(continued)}{\bf .}
        {#2}{\qed}
        }
        
% \renewcommand{\theequation}{\thesection.\arabic{equation}}
% \renewcommand{\thefigure}{\thesection.\arabic{figure}}
% \renewcommand{\thetable}{\thesection.\arabic{table}}
% \newcommand{\Section}[1]{\section{#1}%
%    \setcounter{equation}{0}\setcounter{figure}{0}\setcounter{table}{0}%
%    \setcounter{example}{0}}


%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%
%%%%% TIOA STUFF %%%%%
%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%



% EXECUTIONS TRACES and FRAGS
\newcommand{\extb}[1]{\relax\ifmmode {\sf ExtBeh}_{#1} \else ${\sf ExtBeh}_{#1}$\fi} 
\newcommand{\tdists}[1]{\relax\ifmmode {\sf Tdists}_{#1} \else ${\sf Tdists}_{#1}$\fi} 

\newcommand{\exec}[1]{\relax\ifmmode {\sf Execs}_{#1} \else ${\sf Exec}_{#1}$\fi} 
\newcommand{\execf}[1]{\relax\ifmmode {\sf Execs}^*_{#1} \else ${\sf Exec}^*_{#1}$\fi} 
\newcommand{\execi}[1]{\relax\ifmmode {\sf Execs}^\omega_{#1} \else ${\sf Exec}^\omega_{#1}$\fi} 

\newcommand{\ctrace}[1]{\relax\ifmmode {\sf Ctraces}_{#1} \else ${\sf Ctraces}_{#1}$\fi} 

\newcommand{\trace}[1]{\relax\ifmmode {\sf Traces}_{#1} \else ${\sf Traces}_{#1}$\fi} 
\newcommand{\tracef}[1]{\relax\ifmmode {\sf Traces}^*_{#1} \else ${\sf Traces}^*_{#1}$\fi} 
\newcommand{\tracei}[1]{\relax\ifmmode {\sf Traces}^\omega_{#1} \else ${\sf Traces}^\omega_{#1}$\fi} 

\newcommand{\frag}[1]{\relax\ifmmode {\sf Frags}_{#1} \else ${\sf Frags}_{#1}$\fi} 
\newcommand{\fragf}[1]{\relax\ifmmode {\sf Frags}^*_{#1} \else ${\sf Frags}^*_{#1}$\fi} 
\newcommand{\fragi}[1]{\relax\ifmmode {\sf Frags}^\omega_{#1} \else ${\sf Frags}^\omega_{#1}$\fi} 

\newcommand{\reach}[1]{\relax\ifmmode {\sf Reach}_{#1} \else ${\sf Reach}_{#1}$\fi} 
\newcommand{\pair}[2]{\relax\ifmmode \langle #1, #2 \rangle \else $\langle #1, #2 \rangle$\fi} 

\newcommand{\TE}{\relax\ifmmode \mathit{Time} \else $\mathit{Time}$ \fi} 
\newcommand{\EQ}{\relax\ifmmode \mathit{Enq} \else $\mathit{Enq}$ \fi} 
\newcommand{\DQ}{\relax\ifmmode \mathit{Deq} \else $\mathit{DeqTime}$ \fi} 
\newcommand{\E}{\relax\ifmmode \mathsf{E} \else $\mathsf{E}$ \fi}

\newcommand{\loc}{\relax\ifmmode \mathit{loc} \else $\mathit{loc}$ \fi}
\newcommand{\abs}{\relax\ifmmode \mathit{abs} \else $\mathit{abs}$ \fi}

\newcommand{\execs}{{\exec{}}}
\newcommand{\traces}{{\trace{}}}
\newcommand{\fragss}{{\frag{}}}
\newcommand{\fexecs}{{\execf{}}}
\newcommand{\ftraces}{{\tracef{}}}
\newcommand{\ffragss}{{\fragf{}}}
\newcommand{\iexecs}{{\execi{}}}
\newcommand{\itraces}{{\tracei{}}}
\newcommand{\ifragss}{{\fragi{}}}
\newcommand{\fstate}{{\sf fstate}}  
\newcommand{\lstate}{{\sf lstate}}  
\newcommand{\ltime}{{\sf ltime}}  
\newcommand{\dur}{{\sf dur}}  
\newcommand{\mode}{{\sf mode}}  
\newcommand{\ftime}{{\sf ftime}}  

% 
% \newenvironment{anotation}[1][Nancy]{\begin{quote}\small[[[#1]]]}{\normalsize\end{quote}}
% \newcommand{\ba}{\begin{anotation}}
% \newcommand{\ea}{\end{anotation}}
% 
% \newcommand{\bcb}{\chgbarbegin}
% \newcommand{\ecb}{\chgbarend}
% \chgbarwidth 1pt
% 
% \newcommand{\dec}{\ensuremath{{:}}}
% \newcommand{\eqdef}{\mathbin{::=}}
% \newcommand{\I}{{\ensuremath{\cap}}}



% OPERATIONS ON SETS, RELATIONS AND FUNCTIONS
\newcommand{\pow}[1]{{\bf P}(#1)} % powerset
\newcommand{\inverse}[1]{#1^{-1}}
\newcommand{\range}[1]{\ms{range{(#1)}}}
\newcommand{\domain}[1]{{\it dom}(#1)}
\newcommand{\type}[1]{\ms{type{(#1)}}}
\newcommand{\dtype}[1]{\ms{dtype{(#1)}}} % dynamic type
\newcommand{\restr}{\mathrel{\lceil}}
\newcommand{\proj}{\matrel{\lceil}}
\newcommand{\restrrange}{\mathrel{\downarrow}}
\newcommand{\point}[1]{\wp(#1)}                 %point trajectory



% HYBRID AUTOMATA
\def\A{{\cal A}} % HA
\def\B{{\cal B}} % HA
\def\C{{\cal C}} % HA
\def\D{{\cal D}} % set of discrete steps
\def\E{{\cal E}} % HA
\def\F{{\cal F}} % HA
\def\G{{\cal G}} % pieces of SHIOA
\def\H{{\cal H}} % HA
\def\I{{\cal I}} % environment sequence
\def\K{{\cal K}} % environment sequence
\def\L{{\cal L}} % environment sequence
\def\M{{\cal M}} % Mode switching transitions
\def\O{{\cal O}} % outcome function
\def\P{{\cal P}} % set of modes
\def\Q{{\cal Q}} % set of modes
\def\R{{\cal R}} % relation
\def\S{{\cal S}} % set of trajectories
\def\T{{\cal T}} % set of trajectories
\def\V{{\cal V}} % Lyapunov function
\def\U{{\cal U}} % set of trajectories
\def\X{{\cal X}} % Lyapunov function
\def\Y{{\cal Y}} % set of trajectories
\def\Z{{\cal Z}} % set of trajectories

\def\u{{\mathsf u}} % set of inputs

% more special characters

\newcommand{\col}[1]{\relax\ifmmode \mathscr #1\else $\mathscr #1$\fi}
\def\statemodels{\col{S}}


% Names of actions, automata etc
\definecolor{HIOAcolor}{rgb}{0.776,0.22,0.07}
\newcommand{\HIOA}{\textcolor{HIOAcolor}{\tt HIOA\hspace{3pt}}}
\newcommand{\PVS}{\textcolor{HIOAcolor}{\tt PVS\hspace{3pt}}}
\newcommand{\PVSnogap}{\textcolor{HIOAcolor}{\tt PVS\hspace{1pt}}}
\newcommand{\HIOAbiggap}{\textcolor{HIOAcolor}{\tt HIOA\hspace{6pt}}}
\newcommand{\HIOAnogap}{\textcolor{HIOAcolor}{\tt HIOA}}
\newcommand{\anyrelation}{\lessgtr}

% Transformation for ADT
\newcommand{\SC}[2]{\relax\ifmmode {\tt Scount}(#1,#2) \else ${\tt Scount}(#1,#2)$\fi} 
\newcommand{\SCM}[2]{\relax\ifmmode {\tt Smin}(#1,#2) \else ${\tt Smin}(#1,#2)$\fi} 
\newcommand{\Aut}[1]{\relax\ifmmode {\tt Aut}(#1) \else ${\tt Aut}(#1)$\fi} 

\newcommand{\auto}[1]{{\operatorname{\mathsf{#1}}}}
\newcommand{\act}[1]{{\operatorname{\mathsf{#1}}}}
\newcommand{\smodel}[1]{{\operatorname{\mathsf{#1}}}}
\newcommand{\pvstheory}[1]{{\operatorname{\mathit{#1}}}}
%\newcommand{\auto}[1]{\relax\ifmmode \sf #1\else $\sf #1$\fi}
%\newcommand{\act}[1]{\relax\ifmmode \sf #1\else $\sf #1$\fi}


\newcommand{\Automaton}{{\bf automaton}}
\newcommand{\Asserts}{{\bf asserts}}
\newcommand{\Assumes}{{\bf assumes}}
\newcommand{\Backward}{{\bf backward}}
\newcommand{\By}{{\bf by}}
%\newcommand{\Case}{{\bf case}} -- here
\newcommand{\Choose}{{\bf  choose}}
\newcommand{\Components}{{\bf components}}
\newcommand{\Const}{{\bf const}}
\newcommand{\Converts}{{\bf converts}}
\newcommand{\Do}{{\bf do}}
\newcommand{\Eff}{{\bf eff}}
%\newcommand{\Else}{{\bf else}} -- here
\newcommand{\Elseif}{{\bf elseif}}
\newcommand{\Enumeration}{{\bf enumeration}}
\newcommand{\Ensuring}{{\bf ensuring}}
\newcommand{\Exempting}{{\bf exempting}}
\newcommand{\Fi}{{\bf fi}}
%\newcommand{\For}{{\bf for}} -- here
\newcommand{\Forward}{{\bf forward}}
\newcommand{\Freely}{{\bf freely}}
\newcommand{\From}{{\bf from}}
\newcommand{\Generated}{{\bf generated}}
\newcommand{\Local}{{\bf local}}
\newcommand{\Hidden}{{\bf hidden}}
%\newcommand{\If}{{\bf if}}  -- here
\newcommand{\In}{{\bf in}}
\newcommand{\Implies}{{\bf implies}}
\newcommand{\Includes}{{\bf includes}}
\newcommand{\Introduces}{{\bf introduces}}
\newcommand{\Input}{{\bf input}}
\newcommand{\Kind}{{\bf kind}}
\newcommand{\Initially}{{\bf initially}}
\newcommand{\Internal}{{\bf internal}}
\newcommand{\Invariant}{{\bf invariant}}
\newcommand{\Od}{{\bf od}}
\newcommand{\Of}{{\bf of}}
\newcommand{\Output}{{\bf output}}
\newcommand{\Partitioned}{{\bf partitioned}}
\newcommand{\Pre}{{\bf pre}}
\newcommand{\Signature}{{\bf signature}}
\newcommand{\Simulation}{{\bf simulation}}
\newcommand{\Sort}{{\bf sort}}
\newcommand{\States}{{\bf states}}
\newcommand{\Tasks}{{\bf tasks}}
\newcommand{\Then}{{\bf then}}
\newcommand{\To}{{\bf to}}
\newcommand{\Trait}{{\bf trait}}
\newcommand{\Traits}{{\bf traits}}
\newcommand{\Transitions}{{\bf transitions}}
\newcommand{\Tuple}{{\bf tuple}}
\newcommand{\Type}{{\bf type}}
\newcommand{\Union}{{\bf union}}
\newcommand{\Uses}{{\bf uses}}
\newcommand{\Where}{{\bf where}}
%\newcommand{\While}{{\bf while}} -- here
\newcommand{\With}{{\bf with}}

% Spacing
\newcommand{\FFF}{\vspace{0.1in}}
\newcommand{\BBB}{\hspace{-0.1in}}


